Structured Learning of Two-Level Dynamic Rankings

For ambiguous queries, conventional retrieval systems are bound by two conflicting goals. On the one hand, they should diversify and strive to present results for as many query intents as possible. On the other hand, they should provide depth for each intent by displaying more than a single result. Since both diversity and depth cannot be achieved simultaneously in the conventional static retrieval model, we propose a new dynamic ranking approach. Dynamic ranking models allow users to adapt the ranking through interaction, thus overcoming the constraints of presenting a one-size-fits-all static ranking. In particular, we propose a new two-level dynamic ranking model for presenting search results to the user. In this model, a user's interactions with the first-level ranking are used to infer this user's intent, so that second-level rankings can be inserted to provide more results relevant for this intent. Unlike for previous dynamic ranking models, we provide an algorithm to efficiently compute dynamic rankings with provable approximation guarantees for a large family of performance measures. We also propose the first principled algorithm for learning dynamic ranking functions from training data. In addition to the theoretical results, we provide empirical evidence demonstrating the gains in retrieval quality that our method achieves over conventional approaches.

==> discussion.tex <==

\section{Discussion}


 Another advantage the two-level model has over the static model is that it effectively enables exploration within a topic as well.
 This can be obtained by placing in the first-level ranking, documents having a general, more coarse-grained intent, while having documents in the second-level ranking be oriented towards more specifc intents.
 This is related to the concept of users with the same higher-level intent, but with different specific intents \cite{teev:05}.
 For the query \emph{svm}, having a first-level document on the general intent of the machine learning method, could help guide all users who were specifically looking for either some code, tutorials or a book.
 The model is general enough to work with different granularity of user intents. 


% The {\bf average depth@k} of a ranking  is defined to be the number of relevant documents  (in the top k documents), averaged over all users.
% 
% 
% 
%  It is not hard to show the potential benefit of a two-level ranking via the following observation
% 
% %% <Q2K> I am not sure I understood the precise meaning of this observation. optimal value = ?
% \begin{observ}
% 
% 
%  
%  For a given multi-intent query, we define the Depth Gain as the ratio of the average depth@k for the best two-level ranking , to the average depth@k for the best static ranking.
% %  For a given multi-intent query, let the optimal value across all static rankings of length $k$, for the number of relevant documents, averaged over all users, be $n$. Then the same value across all two-level rankings of length $k$ and width $W$ $(\leq$ $k)$, is as high as $n \times \Big(W - \frac{W(W-1)}{2k}   \Big)$.
% \end{observ}
% 
%  This can easily be seen in the simple example of a query with $k$ different non-overlapping user intents all of which are equally likely.
%  A static ranking of length $k$, would lead to 1 relevant document on average per user.
%  However the dynamic ranking, with the second-level rankings containing results of the same intent as the corresponding head document, leads to an average of $\Big(W - \frac{W(W-1)}{2k}   \Big)$ relevant documents per user.
% 


 We can also show that the best possible $Recall@k$ value across all two-level rankings of length $k$ and width $W$ $(\leq$ $k)$  to be upto  $\Big(W - \frac{W(W-1)}{2k}   \Big)$ times the best $Recall@k$ value across all static rankings of length $k$.
 A similar result holds for $Precision@k$, while the same values for $AP@k$ and $DCG@k$ for two-level rankings are $\Theta(W^2)$ as good as the best values for static rankings.



